A Survey on Robotics with Foundation Models: toward Embodied AI

While the exploration for embodied AI has spanned multiple decades, it remains a persistent challenge to endow agents with human-level intelligence, including perception, learning, reasoning, decision-making, control, and generalization capabilities, so that they can perform general-purpose tasks in open, unstructured, and dynamic environments. Recent advances in computer vision, natural language processing, and multi-modality learning have shown that the foundation models have superhuman capabilities for specific tasks. They not only provide a solid cornerstone for integrating basic modules into embodied AI systems but also shed light on how to scale up robot learning from a methodological perspective. This survey aims to provide a comprehensive and up-to-date overview of foundation models in robotics, focusing on autonomous manipulation and encompassing high-level planning and low-level control. Moreover, we showcase their commonly used datasets, simulators, and benchmarks. Importantly, we emphasize the critical challenges intrinsic to this field and delineate potential avenues for future research, contributing to advancing the frontier of academic and industrial discourse.

==> 02-code-gen.tex <==
% \section{Code Generation with LLM}
% As the LLM has unfolded the capability of  code generation, using LLM to directly generate target code has been a promising domain. In Robotics, works concerning code generation can be broadly categorized into three types:
% policy code, reward code and data generation code. First of all, policy code can be simply seemed as a more detailed task planning which actually transfer the natural language to concrete program. Secondly, reward code means
% using LLM to design the reward function which can be applied in the Reinforcement Learning Framework. Finally, another work trying to use LLM to automatically generate programs contributing to construct trajectories.

% \subsection{Policy Code}
% % Robots need policy to determine what to do next based on the situation. In general, researchers trained a policy model which takes states, images and other information and outputs an action vector directly control the robot. However, policy code is kind of a detailed task planning which actually transfer the natural language to concrete program rather than output the final action vector.
% % Robots using language need it to be grounded to reference the physical world and bridge the connections between words, percepts and actions.And code can describe the spatial position of an object accurately and inform the concrete action such as move, pick.Also using code as a high-level plan has the benefit of expressing functions or feedback loops that process perception outputs and parameterize control primitive APIs.
% Policy code decouples natural language instructions into several steps in code form. Notably, policy code is a well-organized and order sensitive program which involves intricate planning. 
% Grounding portrays a crucial role which establish connections between words, perceptions, and actions. Code, in this context, excels at providing accurate description of the spatial position and exclusive reference of objects. Moreover, employing code as a high-level plan offers the advantage of expressing functions or feedback loops that process perception outputs and parameterize control primitive APIs.

%  CaP\cite{liang2023code} first presented Code as Policies which is a robotic-centric formulation of language model generated programs(LMPs) executed on real systems. With sophisticated prompt engineering, CaP could establish a target program according to the natural language instruction and recursively define new functions to generalize to novel tasks. Indeed, CaP has proposed a highly detailed paradigm for guiding LLM through prompts, while researchers are increasingly focused on its practical application. Following this,\cite{xu2023tool,huang2023audio,vemprala2023chatgpt,liang2023code,zentner2023conditionally,xu2023creative,skreta2023errors,lin2023gesture,mees2023grounding,huang2023instruct2act,parakh2023lifelong,liang2023taskmatrix,li2023interactive,tpvqa2023} prompting LLM to synthesis policy code and they mainly treat the LLM as a high-level planning module. OEIEA\cite{sarch2023open} equips LLM with an external memory of language and program pairs to retrieve in-context examples which are embedded into prompts during LLM querying for novel task plans. ProgPrompt\cite{singh2023progprompt} and Statler\cite{yoneda2023statler} encoded the world state into natural language and then embeded it in prompt for LLM to grounding the action to the physical world.

% \subsection{Reward Code}
% A reward function is a key concept in reinforcement learning, utilized to quantify and measure the behavior of agents in an environment. It defines the feedback from the environment to the agent after it performs a specific action, usually represented as a numerical value. This value can be seen as a measure of the quality of the action, indicating either a reward or a penalty. While designing reward functions is a longstanding challenge in reinforcement learning (RL); it requires specialized knowledge or domain data, leading to high costs for development. So some researchers delegated the LLM to design reward functions in code form that we referred to reward code which significantly reduces human involvement.

% LRRSS\cite{yu2023language} introduce a new paradigm that harnesses this realization by utilizing LLMs to define reward parameters that can be optimized and accomplish variety of robotic tasks.EUREKA\cite{ma2023eureka} introduce Evolution-driven Universal REward Kit for Agent, which takes unmodified environment source code and language task description as context to zero-shot generate executable reward functions from a coding LLM. TEXT2REWARD\cite{xie2023text2reward} introduced a data-free framework that automates the generation of dense reward functions based on LLMs, which can be iterative refined with human feedback. 

% \subsection{Data Generation Code}
% Achieving general-purpose robotic policies necessitates significant amounts of data, which is labor-intensive to collect in the real world. Although simulation provides an economical solution for generating data, there still remains challenges with respect to data diversity. LLMs are involved in data generation by directly loading resources, setting goals and organizing into programs.

% GenSim\cite{wang2023gensim} propose to automatically generate rich simulation environments and expert demonstrations by exploiting an LLM's grounding and coding ability.GenSim introduces goal-directed mode that aims to generate desired tasks and exploratory mode that aims to create novel tasks. SUDD\cite{ha2023scaling} presents a framework which efficiently scale up data generation of language-labelled robot data and effectively distills this data down into a robust multi-task language-conditioned visuomotor policy. LLM acts as a detector to determine whether the trajectory is successful by generating success conditional code.



==> 03-4-data-aug.tex <==
\subsection{Data Augmentation}
\label{sec:data_aug}

The ultimate goal of training an embodied AI policy is to enable that agent to perform a wide variety of different tasks, 
as well as being able to generalize to different scenarios, such as in each person's home, where the furniture and the layout are different in each home.
An essential requirement for this goal is large-scale data, as it has been verified in the training process for large vision and language foundation models.
For embodied AI tasks in the real world, collecting large-scale training data is much more difficult and costly than for vision and language tasks, where large internet-scale data can be collected from many sources like YouTube and Wiki.
During data collection, people need time-consuming training to become proficient in the use of teleoperation equipment and are susceptible to a variety of interfering factors that can lead to mistakes, such as fatigue and distracting events.
Therefore, how to effectively augment the robotic dataset and scale up robot learning is an unavoidable question.

One straightforward approach is to enhance the image data from the perspective of computer vision, which uses commonly used data augmentation techniques, 
such as modifying brightness, flipping, cropping, noise injection, etc. 
However, these methods may destroy the semantic information in the images, which degrades the final performance. 
Recently, data augmentation methods without destroying the semantic information have been proposed to enhance the generalization performance of the policy further by utilizing VLMs and LLMs. 
One of these encouraging works, ROSIE~\cite{yu2023scaling}, reformulates the data augmentation problem as an image inpainting problem. 
It uses the VLMs to delineate the task-relevant region of the images and uses the Imagen Editor, a state-of-the-art diffusion model, to augment the region based on textual instructions. 
Finally, the robot manipulation policy trained on the augmented data shows enhanced generalization capabilities on hundreds of tasks.
% ROSIE~\cite{yu2023scaling} xxx.
% \textbf{Data Augmentation Generation}
% In robot learning, data augmentation and generation are key to overcoming the challenges of collecting extensive datasets. 
% Thanks to the powerful generative capabilities in the foundation models, many methods like ROSIE~\cite{yu2023scaling}, GenAug~\cite{chen2023genaug}, CACTI~\cite{mandi2022cacti}, and DALL-E-Bot~\cite{kapelyukh2023dall} utilize generative models to enrich real-world datasets directly, enhancing policy effectiveness in novel scenarios. 
% % ASSIST~\cite{zhong2023assist} offers a neural rendering simulator for interactive 3D scene editing. 
% In simulators, tools like Gen2Sim~\cite{katara2023gen2sim}, RoboGen~\cite{wang2023robogen}, GenSim~\cite{wang2023gensim}, SUDD~\cite{ha2023scaling}, and MimicGen~\cite{mandlekar2023mimicgen} automate the creation of diverse robotic skills and datasets with minimal human oversight.
% For bridging the sim-to-real gap, methods like domain randomization (DR)~\cite{tobin2017domain}, CPD~\cite{kadokawa2023cyclic}, COMPASS~\cite{huang2023went}, KF~\cite{dong2023kalman}, and PixLDA~\cite{qian2023pixel} are employed.
% to align simulators with real-world environments. 
% TWIST~\cite{yamada2023twist}, HIB~\cite{he2023privileged}, and LHRH~\cite{christen2023learning} further enhance this fidelity. 
% In data generation code, approaches like GenSim~\cite{wang2023gensim} and SUDD~\cite{ha2023scaling} leverage LLMs for efficient and diverse data creation, crucial for developing robust multi-task, language-conditioned visuomotor policies. 
% These advancements collectively signify a substantial leap in robot learning, enabling robots to handle a wider range of tasks and adapt to new environments.

% \textbf{Learning from Human Video}

% %% BC + robot demo, human video + inverse dynamic
% \cite{kim2023giving} trains policies from an eye-in-hand view and masks the human hand and robotic end-effector parts in the image to reduce the gap between human and robot morphologies.



% %% predict future + inverse dynamic, BC
% PLEX~\cite{thomas2023plex} develops a planning-execution architecture based on the transformer model and learns from three types of robotics-relevant data consisting of video-only data, observation-action matching data, and a handful of task-specified expert demonstrations. 

%%

%% representation, compared to MVP, R3M, EgoVLP
% \cite{huo2023human} introduces a multitask learner, Task Fusion Decoder, to learn human-oriented presentations on large video dataset Ego4D~\cite{xx} with a plug-and-play nature that can be adapted to other base models.

==> 04-0-hybrid.tex <==
\section{Foundation Models for Hierarchical Learning}

Current robot learning has achieved unprecedented success on simple tasks such as grasping and placing objects. 
% However, for long distance tasks, training a good network is still very difficult.
However, for long-horizon tasks, such as object rearrangement, learning a single policy is very difficult because errors accumulate quickly with steps.
Most of the approaches can be subsumed into a hierarchical learning framework, where the whole task is divided into many segments at the high level, and each segment is a subtask corresponding to a skill. 
For each subtask, the low-level skill function is then called to accomplish it.
% ~\cite{Ross2010efficient}.
Nevertheless, many planning methods that use only pre-defined primitive tasks (skills) can not generalize to new tasks, which is a prerequisite for robots to be successfully deployed in real-world applications.
Therefore, it is important to learn high-level planning and low-level control simultaneously and make them collaborate seamlessly.
% Here, we use hierarchical learning to refer to algorithms that involve both levels.

Many previous works
% ~\cite{mandlekar2020iris,lynch2020learning,shiarlis2018taco} 
study how to decompose complex tasks rationally and learn corresponding skills effectively.
At present, the development of vision and language foundation models also provides a strong boost to this direction, for example, using LLMs for more rational planning and expanding the skill library.
More specifically,
%% skill, learn from video
% XSkill~\cite{xu2023xskill} learns skill prototypes from unlabeled videos, maps the learned skills into robot actions with diffusion policies, and chains the skills together to solve new tasks.
% %% transformer, skill, both high-level skills and low-level actions
given the high-dimensional visual observation history as the input, Skill Transformer~\cite{huang2023skill} predicts both high-level skills and low-level actions concurrently.
It consists of a skill prediction module and a transformer-based policy that can model the long-horizon sequences and dependencies without making every subtask completely isolated. 
% Thus, it can perform well on long-horizon object rearrangement tasks with unknown noise and new scenarios.
% Skill Transformer~\cite{huang2023skill} takes the high-dimensional visual observation history as the input for a transformer-based policy to predict both high-level skills and low-level actions concurrently.
% %% skill, diffusion, data collect,
Another work is~\cite{ha2023scalingup}, which proposes a skill acquisition framework including a data collection process that generates new trajectories and a distillation process that learns a multi-task visuomotor policy.
To improve the diversity and richness of the generated manipulation trajectories, LLMs provide high-level planning and the success conditions for failure detection and recovery in the form of the code snippet. 
Then, these skills are distilled into a diffusion-based policy to accomplish various tasks.
% with a language-based task planner and a diffusion-based policy into which these skills are distilled.
% % %% human video, high-level plan, low-level control
% MimicPlay~\cite{wang2023mimicplay} proposes a hierarchical framework that learns a goal-conditioned latent planner and a low-level controller from two data sources, including human play data and robot demonstrations.
% %% skill,  LLMs
% BOSS~\cite{zhang2023bootstrap} escalates the set of primitive skills and fills the skill library by chaining different meaningful skills together using LLMs.
% %% skill, continual learning
% % SANER~\cite{powers2023evaluating} improves upon the SANE method~\cite{xx} and continually expands the skill set from demonstrations of different tasks in the continual learning setting for a real-world home robot.
% SANER~\cite{powers2023evaluating} continually expands the skill set from demonstrations of different tasks in the continual learning setting for a real-world home robot.
% % %% RL, locomotion skill: rolling, walking, standing
% % \cite{meng2023rolling} devises a novel multi-path reward function in RL to enable humanoid robots to acquire motor skills from rolling over to walking.
% % %% LLMs, reward function, MPC
% % \cite{yu2023language} converts task descriptions into reward functions by utilizing the code-writing ability of LLMs and then uses model predictive control (MPC) methods to synthesize low-level robot actions.
% %% LLMs, planning, skill ~\cite{simeonov2022neural}
% \cite{parakh2023lifelong} teaches robots new skills in the continual learning setting by using LLMs as the planner to query new skills and use Neural Descriptor Fields (NDFs) as the skilled executor. 
% % %% VLMs, instruction augmentation
% % DIAL~\cite{xiao2022robotic} uses CLIP~\cite{radford2021learning} to augment instructions, injects semantic knowledge into the large-scale unlabeled dataset, and then trains a language-conditioned policy.
% %% pre-training, LLMs, skill, rejected by ICLR23
% SPRINT~\cite{zhang2023sprint} designs instruction relabelling and cross-trajectory skill chaining using LLMs to reduce laborious costs and implements a scalable offline policy pre-training method.

% %%%%%%%%%%%%%%%%%%%%%%%
% \textbf{Planning}

% %% itself as a foundation model, planning, use RT-1 as low-level
% PaLM-E~\cite{driess2023palm} introduces a general-purpose behemoth model with 562B parameters for various visual, language, and embodied reasoning tasks.

% %% reasoning, planning, dataset
% ~\cite{kwon2023toward} enables agents to actively explore and perceive information from environments by querying LLMs and VLMs.
% This work also releases the MESSYSURFACES dataset, which contains 70 real-world surfaces for surface tidying tasks.

% %% planning, LLMs, low-level
% \cite{cao2023ground} focuses on the planning-to-execution transition problem and designs a prompt that enables LLMs to generate low-level actions given a robotic primitive task description.

% %% diffusion, subgoal planning, pre-trained model
% SuSIE~\cite{black2023zero} fine-tunes a pre-trained diffusion-based image-editing model to predict subgoals for low-level control policy, which is trained in a supervised manner. 

% %% LLMs, planning, skill
% Text2Motion~\cite{xx} tackles long-horizon manipulation tasks by assessing the feasibility of the skill sequences according to the Q-values of the skills and guiding the planning generation from LLMs.


==> 05-data-aug.tex <==
% \section{Data Augmentation Generation}

% Recent strides in robot learning hold great potential for empowering robots to execute diverse manipulation tasks and adapt to unfamiliar scenarios. A pivotal element driving this advancement is the scale of robot data utilized for model training. Previous methods for acquiring extensive datasets have depended on either demonstrations that demand significant human engagement or intricate autonomous data collection strategies that are burdensome to scale.
% \subsection{Real-Data Augmentation}

% Training an agent using extensive robot data is a viable method, yet expanding real-world data doesn't match the rapid growth seen in fields like natural language processing (NLP) or computer vision (CV). This slower growth is due to the need for deploying numerous costly devices for data collection, significantly limiting the expansion of real-world robotic data. Consequently, many researchers are exploring the use of current generative models to enrich data from real-world scenarios.
% To tackle the challenge of large-scale data scarcity, \textbf{ROSIE}\cite{yu2023scaling} illustrates that the application of text-to-image diffusion models to existing robotic manipulation datasets can enhance policy effectiveness in novel scenarios, such as those involving unfamiliar objects and distractors.
% Similarly,\textbf{GenAug}\cite{chen2023genaug} shows using generative models to create “augmented” RGBD images for entirely different and realistic environments, and retarget behaviors to new scenarios.
% \textbf{CACTI}\cite{mandi2022cacti}shows using generative models like stable diffusion to add distractors of the scene can robustify the multi-task policy learning.
% \textbf{DALL-E-Bot}\cite{kapelyukh2023dall}: Introducing Web-Scale Diffusion Models to Robotics by Kapelyukh et al leverages DALL-E to generate goal images for rearrangement tasks.

% \textbf{ASSIST}\cite{zhong2023assist},an object-wise neural rendering simulator equipped with interactive 3D scene editing capabilities.



% \subsection{Sim-Data Generation}

% Robot data sets in real scenarios are relatively difficult to obtain, so some researchers hope to improve the capabilities of agents by expanding the scale of simulation data sets. for example,

% \textbf{Gen2Sim}\cite{katara2023gen2sim} transforms 2D images into 3D assets, assembles scenes, and uses LLMs to generate detailed task descriptions and sub-tasks.

% \textbf{RoboGen} \cite{wang2023robogen}and  \textbf{scalingup} \cite{ha2023scalingup}  are automated systems that employ generative simulation and cutting-edge LLM technologies to develop and acquire a broad spectrum of robotic skills.
% % It generates tasks, scenes, and training supervisions with minimal human oversight, marking a significant step towards scalable robotic skill learning in simulated environments.
% \textbf{MimicGen} \cite{mandlekar2023mimicgen}is a system designed for automatically generating extensive and detailed datasets using a minimal number of human demonstrations. It achieves this by adapting the provided demonstrations to new contexts, resulting in large-scale, rich datasets for training.


% \subsection{Sim-to-Real}
% % \subsubsection{domain randomization}
% There is still a gap between the actions predicted by the agent trained by the simulator and deployed in the real world, and some enhanced methods are still needed to bridge the gap between the simulator and the real world. Some common sim-to-real methods include domain randomization, distillation, image segmentation, etc. for example,CPD\cite{kadokawa2023cyclic} strategically partitions the range of randomized parameters into smaller sub-domains, each associated with a dedicated local policy. The learning process involves cyclic transitions between these sub-domains. \textbf{COMPASS} \cite{huang2023went} aligns the simulator with the real world by uncovering the causal relationship between the environment parameters and the simulation-to-reality gap.\textbf{KF} \cite{dong2023kalman}it treats the gap between the real physical environment and the simulated environment as a Gaussian perturbation, it utilizes Kalman filtering to reduce the discrepancy.\textbf{PixLDA}\cite{qian2023pixel} proposes a pixel-level domain adaptation (Pixel-DA), a real-to-sim approach for unsupervised domain adaptation in object pose estimations.\textbf{TWIST }\cite{yamada2023twist}(Teacher-Student World Model Distillation for Sim-to-Real Transfer) to achieve efficient sim-to-real transfer of vision-based model-based RL using distillation.\textbf{HIB }\cite{he2023privileged,}learns a privileged knowledge representation from historical trajectories by capturing the underlying changeable dynamic information.Learning Inertial Parameter Identification of Unknown Object with Humanoid Robot using Sim-to-Real Adaptation \cite{baek2023learning} enhance the fidelity of the simulation by Robot System Identification (SysID) and Gaussian Processes.\textbf{CycleGAN} \cite{shi2023sim}introduce a domain adaptation method utilizing CycleGAN and a force control transfer approach to address the reality gap.\textbf{LHRH }\cite{christen2023learning} propose a two-stage teacher-student framework incorporating motion and grasp planning, reinforcement learning, and self-supervision, trained with human-in-the-loop.

% %% data generation code
% \subsection{Data Generation Code}
% Achieving general-purpose robotic policies necessitates significant amounts of data, which is labor-intensive to collect in the real world. Although simulation provides an economical solution for generating data, there still remains challenges with respect to data diversity. LLMs are involved in data generation by directly loading resources, setting goals and organizing into programs.

% GenSim\cite{wang2023gensim} propose to automatically generate rich simulation environments and expert demonstrations by exploiting an LLM's grounding and coding ability.GenSim introduces goal-directed mode that aims to generate desired tasks and exploratory mode that aims to create novel tasks. SUDD\cite{ha2023scaling} presents a framework which efficiently scale up data generation of language-labelled robot data and effectively distills this data down into a robust multi-task language-conditioned visuomotor policy. LLM acts as a detector to determine whether the trajectory is successful by generating success conditional code.

